Automaton-Based Representations of Task Knowledge from Generative Language Models

Automaton-based representations of task knowledge play an important role in control and planning for sequential decision-making problems. However, obtaining the high-level task knowledge required to build such automata is often difficult. Meanwhile, large-scale generative language models (GLMs) can automatically generate relevant task knowledge. However, the textual outputs from GLMs cannot be formally verified or used for sequential decision-making. We propose a novel algorithm named GLM2FSA, which constructs a finite state automaton (FSA) encoding high-level task knowledge from a brief natural-language description of the task goal. GLM2FSA first sends queries to a GLM to extract task knowledge in textual form, and then it builds an FSA to represent this text-based knowledge. The proposed algorithm thus fills the gap between natural-language task descriptions and automaton-based representations, and the constructed FSA can be formally verified against user-defined specifications. We accordingly propose a method to iteratively refine the queries to the GLM based on the outcomes, e.g., counter-examples, from verification. We demonstrate GLM2FSA's ability to build and refine automaton-based representations of everyday tasks (e.g., crossing a road), and also of tasks that require highly-specialized knowledge (e.g., executing secure multi-party computation).

==> figures/intro_example_.tex <==


% a screenshot of this was used in the figure

\begin{adjustbox}{width=\linewidth,height=3cm,keepaspectratio}
\noindent\begin{minipage}{46em}
\begin{lstlisting}[language=completion,basicstyle=\fontsize{8}{9}\selectfont]
    <prompt>Steps for: Cross the road
    [1]</prompt><completion> Look both ways before crossing the road.
    [2] If there are no cars coming, proceed to cross the road.
    [3] If there are cars coming, wait for them to pass before crossing the road.</completion>
    
    <prompt>Substeps for: [1] Look both ways before crossing the road.
    [1.1]</prompt><completion> Face the direction you want to cross the road in.
    [1.2] Look to the left.
    [1.3] Look to the right.
    [1.4] If there are no cars coming, proceed to [2]. If there are cars coming, proceed to [3].</completion>
    ...
\end{lstlisting}
\end{minipage}
\end{adjustbox}
